CARING-AI: Towards Authoring Context-aware Augmented Reality INstruction through Generative Artificial Intelligence

Context-aware AR instruction enables adaptive and in-situ learning experiences. However, hardware limitations and expertise requirements constrain the creation of such instructions. With recent developments in Generative Artificial Intelligence (Gen-AI), current research tries to tackle these constraints by deploying AI-generated content (AIGC) in AR applications. However, our preliminary study with six AR practitioners revealed that the current AIGC lacks contextual information to adapt to varying application scenarios and is therefore limited in authoring. To utilize the strong generative power of GenAI to ease the authoring of AR instruction while capturing the context, we developed CARING-AI, an AR system to author context-aware humanoid-avatar-based instructions with GenAI. By navigating in the environment, users naturally provide contextual information to generate humanoid-avatar animation as AR instructions that blend in the context spatially and temporally. We showcased three application scenarios of CARING-AI: Asynchronous Instructions, Remote Instructions, and Ad Hoc Instructions based on a design space of AIGC in AR Instructions. With two user studies (N=12), we assessed the system usability of CARING-AI and demonstrated the easiness and effectiveness of authoring with Gen-AI.

==> texes/1-Introduction-archived.tex <==
\section{Introduction}
%introduction to the background in AR Instruction -> GenAI in other fields brings easiness of content creation -> can we introduce the same easiness in the field of AR Instruction? -> we develop a system to prove our hypothesis/ to make it happen
% Scope: AR Instructions applications 
% JS: I do not wish to be verbose here considering many other items to be talked about in the introduction.
% Thus I removed most of my exemplifying in the first paragraph.
Augmented Reality (AR) instructions provide an interactive and immersive learning experience by rendering digital content onto physical objects or environments and enabling users to visualize complex concepts or procedures, explore various scenarios, and practice skills in a more realistic and context-rich setting.
% (e.g. text~\cite{}, image~\cite{}, video~\cite{}, or audio~\cite{}).
Due to their vast capabilities and their potential to enhance user engagement~\cite{weerasinghe2022arigato}, facilitate learning~\cite{zhu2023learniotvr}, and improve performance~\cite{hoover2020measuring, christopoulos2022effects} in various contexts, AR instructions have gained considerable attention in a range of fields. %, including education~\cite{}, healthcare~\cite{}, and industrial training~\cite{}.

% Existing methodologies: authoring AR instructions: programming (expertise), demonstration (code-less, but hardware, motion needed, single input modality), generative AI (ad hoc, no need for hardware or demonstration, multi-modalities, but need contextual information)
In the domains where AR instructions for human motion are necessary, animated humanoid avatars for AR instructions have been favored and widely applied as an expressive visualization technique~\cite{cao2020exploratory, chidambaram2021processar}.
To author animated humanoid avatars, one can program through keyframe animation or inverse kinematics in development platforms, such as Unity~\cite{unity3d}, Unreal Engine~\cite{unreal_engine}, or Blender~\cite{blender}.
However, these methods have been criticized for their requirement that the author have expertise in both the subject matter of the instructions and the programming for animation~\cite{chidambaram2021processar}.

To overcome the low-level programming criteria for authoring animated humanoid avatars, a promising alternative is authoring through embodied demonstration (i.e. creating or editing digital content in AR environments by physically interacting or demonstrating actions in the real world).
It is proven to enhance the realism~\cite{weidner2023systematic, kim2023avatar}, code-less efficiency in creating~\cite{9994974}, engagement~\cite{alblehai2022individual, morris2020toward, black2017can}, interactions~\cite{wang2020avatarmeeting, jo2015spacetime}, and learning and training gain~\cite{zhu2023learniotvr} in AR instruction applications.
Despite the benefits and simplicity for the authors, authoring by embodied demonstrations is still subject to real-world human motion and hardware requirements for motion capture (Mocap).

The very rapid and exponential development of Generative Artificial Intelligence (Gen-AI) has brought AI-generated content (AIGC) into the discussion of authoring AR instructions~\cite{hu2023exploring}, considering its potential to eliminate expertise barriers and hardware requirements.
With this rapid growth of Gen-AI power, content creation in various modalities can be democratized to higher levels ~\cite{LV2023208, cao2023comprehensive}.
Users are enabled to generate desired content by simply prompting via intuitive modalities (e.g. textual conversation~\cite{radford2018improving, radford2019language, keskar2019ctrl, brown2020language} and reference image~\cite{radford2021learning, ramesh2021zeroshot, ramesh2022hierarchical}).
Many ongoing research and discussions have identified opportunities for the deployment of AIGC in AR for its overwhelming power of abstracting human knowledge and a wide range of I/O modalities~\cite{cao2023comprehensive, shi2023hci}.
In pursuit of the design space of AIGC in AR instructions, some research has pointed out that Gen-AI lacks the contextual and background information to be deployed into real-world applications~\cite{LV2023208}.

% Context information is important in AR instruction. According to prior works, there are three types of contexts: human, environmental, and system. Each serves a purpose in AR instruction.
In the scope of AR instruction, contextual information is a critical metaphor.
A taxonomy of context awareness in AR instruction, that many prior works converge towards, encompasses three key aspects: the human, environment, and system~\cite{qian2023explore, grubert2016towards, wang2022supporting}.
Human context awareness enables the system to provide instructions that are adaptive to the users' profiles~\cite{huang2021adaptutar}, social situation~\cite{davari2022validating} or states~\cite{wang2020capturar, doughty2021surgeonassist, pan2021knowing}.
Environmental context awareness merges the AR instructions with the physical world by considering the physical~\cite{ruizhi2021context, muff2022framework, scargill2021context} and semantic~\cite{chen2020context, gutierrez2018phara, lacoche2022prototyping} information in the environment.
System context depicts the state of the AR systems as well as their I/O, which can be considered when given the next procedural instructions~\cite{yigitbas2019context, yin2018synchronous, seeliger2022context}.
All three aspects of context awareness are essential for grounding AIGC in AR instructional applications.

% To provide such contexts, we come up with our system, to address the problem. Describe the workflow of our system and how it addresses each design consideration of the contexts.
To this end, we aim to investigate the methodology to fill the gap between state-of-the-art Gen-AI and context-aware AR humanoid avatar instructions.
Specifically, our research is motivated to explore (1) What context information does AI-generated humanoid avatar animation lack for AR instructions? (\autoref{sec:designrationale}) (2) How can this missing contextual information be delivered to Gen-AI? and (\autoref{sec:system}) (3) What insights can we gain from our designs to further foster developments towards the use of AIGC in AR? (\autoref{sec:discussion})

From a preliminary expert interview, we summarize the design goals for naturally providing contextual information to AIGC incorporating user interactions in the authoring process.
We then present CARING-AI, an AR system enabling authoring contextualized humanoid avatar animation for AR instructions.
Given a textual description of the task to instruct, CARING-AI generates step-by-step textual instructions that can be modified by the users and further generates motion that animates humanoid avatars as the visual cues in the instructions.
From the authors' customization of the steps and natural interactions such as (a) the authors' perception of humans moving across an environment in a particular context, and (b) the spatial scales of the instructions;  CARING-AI temporally and spatially adapts the AI-generated instructions to the human, environment, and system context of the task.
% First application
% To the best of our knowledge, CARING-AI is the first AR instruction application that creates AI-generated humanoid avatars from text input.
 
% Our contributions: workflow, algorithm, system, and a user study with discussions for further exploratory insights
Our contributions are four-fold:
\begin{itemize}
    \item A code-less and Mocap-free workflow for authoring animated humanoid avatar instructions in AR with Generative-AI that is contextually aware of the human, environment, and system.
    \item A diffusion-model-based algorithm to temporally smooth sequences of individually generated humanoid motions.
    \item An AR interface for authoring AR instructions from textual input describing the tasks, avatars' trajectory, and directional vision.
    \item A user study evaluating our system and workflow along with in-depth discussions for future exploratory directions in the scope of AIGC in AR.
\end{itemize}

==> texes/5-Applications.tex <==
\section{Application Scenario}

\begin{figure}[ht]
    \centering
    \includegraphics[width=.65\textwidth]{figures/case1.png}
    \caption{CARING-AI for authoring asynchronous Instructions. A senior lab researcher (a) leaves an AR memo for his colleague on how to use a 3D printer. He simply walks around the printing lab using CARING-AI to contextualize the textual instructions, capturing the location of the PVA filament and the printer. (b) The corresponding humanoid animation is generated according to the step-by-step instructions. CARING-AI is capable of handling AR instructions of diverse content and context, namely spatial or temporal context, and local or global content.}
    \label{fig:usecase1}
\end{figure}

With CARING-AI, users are enabled to author context-aware humanoid avatar animation for AR instructions that can be adaptively deployed into various application scenarios (\textbf{AS}).
Our primary goal of presenting the \textbf{AS} is to demonstrate that CARING-AI can capture and convey context information identified in design space.
Specifically, we showcase three major scenarios where CARING-AI demonstrates its ability to grant code-less and Mocap-free authoring (\textbf{AS-1}, \textbf{AS-2}, and \textbf{AS-3}), create content that is to be deployed in different time primitives or via different platforms (\textbf{AS-1}, \textbf{AS-3}), and adapt to varying contexts (\textbf{AS-2}).

\subsection{AS-1: Asynchronous Instructions}

Asynchronous instructions are the most common case in the applications of AR instructions, where the authors create the content prior to the consumption of the AR experiences~\cite{chen2023papertoplace, chidambaram2021processar}.
CARING-AI naturally supports asynchronous instructions and situates AI-generated humanoid avatar animation into the physical world contextually.
Here, we showcase a scenario in a research lab, where a senior researcher (Tom, the author) would like to leave an AR memo for his junior colleague (Jerry, the consumer) to instruct him on how to operate a 3D printer.
Tom creates and modifies the text instructions with the help of CARING-AI, then provides context to the system by walking up to the locations and taking snapshots of the environment as shown in ~\autoref{fig:usecase1}.
He informs Jerry to get the printing materials and then go to a specific 3D printer to print a product.
Later, when Jerry arrives in the laboratory, he can see and follow the step-by-step AR memo from Tom to start working on the product.


\begin{figure}[htp]
    \centering
    \includegraphics[width=.75\textwidth]{figures/case2.png}
    \caption{CARING-AI for Ad Hoc AR Instructions. For the same task (e.g. installing a router), the instructions vary across diverse contexts. By using CARING-AI, users simply need to scan the environment to provide contextual information to the system. CARING-AI will generate humanoid avatar animation that blends into different physical realities (e.g. an office, a bedroom, or a living room)}
    \label{fig:usecase2}
\end{figure}


\subsection{AS-2: Ad Hoc Instruction Creation}


CARING-AI enables authoring AR instructions through Gen-AI by contextualizing the instructions.
In this scenario, we showcase how CARING-AI enables authoring ad hoc instructions in changing contexts with simplified user interactions.
As a technician from the lab, Tom would like to teach his colleague how to install a router as shown in ~\autoref{fig:usecase2}.
The instructions are fairly simple and easy to understand.
However, the detail of the steps varies across environments, e.g. in the office, the bedroom, or the living room, because the locations of the router and the outlet vary.
With the same protocol to be visualized, Tom simply has to contextualize the protocol in different places, assigning the locations of the objects by traversing the rooms.
As a result, Tom authors different avatar animations for diverse contexts with the same instruction protocol.

\begin{figure}[htp]
    \centering
    \includegraphics[width=.75\textwidth]{figures/case3.pdf}
    \caption{CARING-AI's capability of authoring Remote Instructions. In this scenario, a delivery man is asking for the destinations of the packages. (a) A lab member is giving contextual information through a pre-scanned scenario in VR. (b) We built a mock-up VR scenario to record the locations and correspond them back into the physical reality. Once the instructions are contextualized, the delivery man can view the humanoid instructions on delivering the packages (c, d).}
    \label{fig:usecase3}
\end{figure}

\subsection{AS-3: Remote Instructions}

In this scenario, CARING-AI is deployed in a remote instruction task.
We showcased how CARING-AI can adapt to context information of diverse modalities and liberate the authors from demonstrating in the actual physical environment.
Toodles, the \deliverywoman of the building, arrives in the lab with new devices to be allocated ~\autoref{fig:usecase3} (c).
Noticing no one is in the lab, \Toodles contacts Jerry, asking about the allocation of the devices.
Jerry, who is not present at the lab, confirms the devices and their checkout points (i.e. where they are to be placed).
Jerry then enters a pre-scanned point-cloud map of the lab in Virtual Reality (VR), where he authors the instructions in VR using CARING-AI by navigating the map and taking screenshots ~\autoref{fig:usecase3} (a, b) (We built a mock-up VR program to record Jerry's locations in VR and correspond them to the physical reality).
CARING-AI generates humanoid avatar instructions according to the contextual information provided.
The authored AR instructions are then sent to \Toodles, who follows the avatar demonstrations to allocate the devices to different locations~\autoref{fig:usecase3} (d, e).
In this case, we see that CARING-AI is capable of authoring synchronous remote instructions.
It also showcases the possibilities of authoring AR experiences in VR with CARING-AI with aligned contextual information between physical reality and VR. The alignment of context is subsumed here as described and inspired by many prior works~\cite{qian2022scalar, Nebeling2020XRDirector, wang2021distanciar}


